On Robustness of Neural Semantic Parsers

Semantic parsing maps natural language (NL) utterances into logical forms (LFs), which underpins many advanced NLP problems. Semantic parsers gain performance boosts with deep neural networks, but inherit vulnerabilities against adversarial examples. In this paper, we provide the empirical study on the robustness of semantic parsers in the presence of adversarial attacks. Formally, adversaries of semantic parsing are considered to be the perturbed utterance-LF pairs, whose utterances have exactly the same meanings as the original ones. A scalable methodology is proposed to construct robustness test sets based on existing benchmark corpora. Our results answered five research questions in measuring the sate-of-the-art parsers' performance on robustness test sets, and evaluating the effect of data augmentation.

==> To_do.tex <==
Substituiton(f)

how mani capit is s0 have	
( count $0 ( and ( capital:t $0 ) ( loc:t $0 s0 ) ) )
( capital:c s0 )
(size:i s0 )
( capital:c s0 )





Substituiton(nf)
what are the main river in s0
( lambda $0 e ( and ( major:t $0 ) ( river:t $0 ) ( loc:t $0 s0 ) ) ) 
( lambda $0 e ( and ( river:t $0 ) ( loc:t $0 s0 ) ) ) 
(lambda $0 (and (river:t $0 ) (loc:t $0 s0 ) ) ) 
( lambda $0 e ( and ( river:t $0 ) ( loc:t $0 s0 ) ) )
what are the major river in s0

back translation
what kind of work do you have with languageid0	
job ( ANS ) , language ( ANS , languageid0 )
job ( ANS ) , application ( ANS , languageid0 )
(answer (job ANS ) (language ANS languageid0 ) (language ANS languageid0 ) )
job ( ANS ) , language ( ANS , languageid0 ) , application ( ANS , languageid0 )


list job use languageid0





==> tab-rq3.tex <==

\begin{table*}[!ht]
\centering
   \resizebox{0.9\textwidth}{!}{%
  \begin{tabular}[t]{|l|c c c|c c c|c c c|}
    \toprule
    \multirow{2}{*}{Generation Methods} &
      \multicolumn{3}{c|}{\Jobs} &
      \multicolumn{3}{c|}{\Geo} &
      \multicolumn{3}{c|}{\Atis} \\
      & \seqseq $\quad$ & \coarsefine $\quad$ & \tranx $\quad$ & \seqseq $\quad$ & \coarsefine $\quad$ & \tranx $\quad$ & \seqseq $\quad$ & \coarsefine $\quad$ & \tranx \\
      \midrule
    Insertion & 7.06/8.55  & 7.04/9.50 &6.72/5.84   & 10.78/8.6  & 8.98/8.88  & 6.32/6.88  & 12.03/2.33  & 4.53/4.98 & 10.83/8.95\\
    Substitution (f) & 13.62/10.49 & 14.73/4.7 & 4.51/5.11 & 13.33/9.72 & 4.89/4.06 &10.10/5.85 & 29.36/16.48 &21.4/13.21  &  24.36/18.92\\

    Deletion & 9.6/8.32 & 3.27/3.93 &13.78/6.14 & 14.39/11.07 & 5.68/4.69 &21.20/6.52  &16.99/13.08  &14.36/10.53  &   34.77/20.74\\
    Substitution (nf) & 6.55/3.60 &2.32/4.41  &5.4/2.9 & 50.86/24.17 &15.44/10.07 &47.36/23.88 & 50.83/26.94 &  20.68/12.87 &   51.48/24.25\\
    \hline
    Back Translation $\,$& 61.97/32.11&42.34/37.83 & 53.88/40.48  & 48.34/30.46 &33.66/27.12 &47.33/29.73   &38.79/26.77 &28.08/18.31  &   45.58/26.17 \\
    Reordering &62.72/50.36  &47.11/37.30  & 42.34/37.83 &66.38/43.19  &48.93/31.27  &60.16/38.30 &38.79/26.77  &28.08/18.31  & 42.07/29.70 \\
    \hline
    Overall(micro) & 20.17/18.79 &11.12/12.84  & 27.00/23.75 & 22.93/21.06 & 14.26/9.98 & 20.49/18.39  & 29.58/21.31 & 14.86/17.62 &14.24/15.59 \\
      Overall(macro) &26.92/18.90  &20.01/14.34  & 17.98/12.944 &34.01/21.20  &18.70/14.37  & 32.08/18.54  & 34.02/21.42 &21.41/14.91  & 36.15/23.8\\
    \bottomrule
  \end{tabular}%
   }
       \vspace{-2mm}
     \caption{Black-box attack successful rate before/after adversarial training }
  \label{tab:rq3}
     \vspace{-2mm}
\end{table*}
                    
